Toward the Verification of a Simple Hypervisor

Virtualization promises significant benefits in security, efficiency, dependability, and cost. Achieving these benefits depends upon the reliability of the underlying virtual machine monitors (hypervisors). This paper describes an ongoing project to develop and verify MinVisor, a simple but functional Type-I x86 hypervisor, proving protection properties at the assembly level using ACL2. Originally based on an existing research hypervisor, MinVisor provides protection of its own memory from a malicious guest. Our long-term goal is to fully verify MinVisor, providing a vehicle to investigate the modeling and verification of hypervisors at the implementation level, and also a basis for further systems research. Functional segments of the MinVisor C code base are translated into Y86 assembly, and verified with respect to the Y86 model. The inductive assertions (also known as "compositional cutpoints") methodology is used to prove the correctness of the code. The proof of the code that sets up the nested page tables is described. We compare this project to related efforts in systems code verification and outline some useful steps forward.

==> eptcsdata.tex <==
\providecommand{\firstpage}{28}
\providecommand{\publicationstatus}{Hardin and Schmaltz (Eds): ACL2 2011\\
EPTCS 70, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.70.3}{10.4204/EPTCS.70.3}}

